On spectrum of the zero-divisor graph of matrix ring

For a ring $R$, the zero-divisor graph is a simple graph $\Gamma(R)$ whose vertex set is the set of all non-zero zero-divisors in a ring $R$, and two distinct vertices $x$ and $y$ are adjacent if and only if $xy=0$ or $yx=0$ in $R$. By using Weyl's inequality we give bounds on eigenvalues of adjacency matrix of $\Gamma(M_2(F))$, where $M_2(F)$ is a $2 \times 2$ matrix ring over a finite field $F$.

==> ref.tex <==

\begin{document}



@article{monius2021eigenvalues,
  title={Eigenvalues of zero-divisor graphs of finite commutative rings},
  author={M{\"o}nius, Katja},
  journal={Journal of Algebraic Combinatorics},
  volume={54},
  pages={787--802},
  year={2021},
  publisher={Springer}
}

@Book{shurcomplement,
  title={Schur Complements and Applications},
  author={J. Gallier },
  pages={431-437},
  year={2011},
  address = {New York},
  publisher={Springer}
}

@book{godsil2001algebraic,
  title={Algebraic graph theory},
  author={Godsil, Chris and Royle, Gordon F},
  volume={207},
  year={2001},
  address = {New York},
  publisher={Springer Science \& Business Media}
}
@Book{weyl,
  title={Inequalities: Theory of Majorization and Its Applications },
  author={ Albert W. Marshall , Ingram Olkin , Barry C. Arnold },
  pages={336},
  year={2011},
  address = {New York},
  publisher={Springer}
}
@Book{dbwest,
  title={Introduction to Graph Theory},
  author={Douglas B. West },
  pages={453-455},
  year={2002},
  address = {India},
  publisher={Pearson Education}
}
@Article{patil2021spectrum,
  title={Spectrum of the zero-divisor graph of von Neumann regular rings},
  author={Patil, Avinash and Shinde, Kiran},
  journal={J. Algebra Appl.},
  pages={2250193},
  year={2021},
  publisher={World Scientific}
}

@article{chattopadhyay2020laplacian,
  title={Laplacian eigenvalues of the zero divisor graph of the ring $\mathbb Z_n$},
  author={Chattopadhyay, Sriparna and Patra, Kamal Lochan and Sahoo, Binod Kumar},
  journal={Linear Algebra Appl.},
  volume={584},
  pages={267--286},
  year={2020},
  publisher={Elsevier}
}

@article{pirzada2021eigenvalues,
  title={On the eigenvalues of zero-divisor graph associated to finite commutative ring},
  author={Pirzada, S and Wani, Bilal A and Somasundaram, A},
  journal={AKCE Int. J. Graphs Comb.},
  volume={18},
  number={1},
  pages={1--6},
  year={2021},
  publisher={Taylor \& Francis}
}

@article{chattopadhyay2020laplacian,
  title={Laplacian eigenvalues of the zero divisor graph of the ring Zn},
  author={Chattopadhyay, Sriparna and Patra, Kamal Lochan and Sahoo, Binod Kumar},
  journal={Linear Algebra Appl.},
  volume={584},
  pages={267--286},
  year={2020},
  publisher={Elsevier}
}

@article{magi2020adjacency,
  title={Adjacency matrix and eigenvalues of the zero divisor graph $\Gamma$ (Zn)},
  author={Magi, PM and Jose, Sr Magie and Kishore, Anjaly},
  journal={J. Math. Comput. Sci.},
  volume={10},
  number={4},
  pages={1285--1297},
  year={2020}
}

@article{anderson1999zero,
  title={The zero-divisor graph of a commutative ring},
  author={Anderson, David F and Livingston, Philip S},
  journal={J. Algebra},
  volume={217},
  number={2},
  pages={434--447},
  year={1999},
  publisher={Elsevier}
}

@article{beck1988coloring,
  title={Coloring of commutative rings},
  author={Beck, Istv{\'a}n},
  journal={J. Algebra},
  volume={116},
  number={1},
  pages={208--226},
  year={1988},
  publisher={Elsevier}
}

@article{patil2017zero,
  title={On the zero-divisor graph of Rickart*-rings},
  author={Patil, Avinash and Waphare, BN},
  journal={Asian-Eur. J. Math.},
  volume={10},
  number={01},
  pages={1750015},
  year={2017},
  publisher={World Scientific}
}

@article{patil2018zero,
  title={The zero-divisor graph of a ring with involution},
  author={Patil, Avinash and Waphare, BN},
  journal={Journal of Algebra and Its Applications},
  volume={17},
  number={03},
  pages={1850050},
  year={2018},
  publisher={World Scientific}
}

@article{akbari2004zero,
  title={On the zero-divisor graph of a commutative ring},
  author={Akbari, S and Mohammadian, A},
  journal={Journal of algebra},
  volume={274},
  number={2},
  pages={847--855},
  year={2004},
  publisher={Elsevier}
}
@article{redmond2002zero,
  title={The zero-divisor graph of a non-commutative ring},
  author={Redmond, Shane P},
  journal={Int. J. Commut. Rings},
  volume={1},
  number={4},
  pages={203--211},
  year={2002}
}

@article{cardoso2013spectra,
  title={Spectra of graphs obtained by a generalization of the join graph operation},
  author={Cardoso, Domingos M and de Freitas, Maria Aguieiras A and Martins, Enide Andrade and Robbiano, Mar{\'\i}a},
  journal={Discrete Mathematics},
  volume={313},
  number={5},
  pages={733--741},
  year={2013},
  publisher={Elsevier}
}

@article{patil2021spectrum,
  title={Spectrum of the zero-divisor graph of von Neumann regular rings},
  author={Patil, Avinash and Shinde, Kiran},
  journal={J. Algebra Appl.},
  pages={2250193},
  year={2021},
  publisher={World Scientific}
}

@article{thakare1998baer,
  title={Baer $*$-Rings With Finitely Many Elements},
  author={Thakare, NK and Waphare, BN},
  journal={J. Comb. Math. Comb. Comput.},
  volume={26},
  pages={161--164},
  year={1998},
  publisher={CHARLES BABBAGE RESEARCH CENTRE}
}


@book{dbwest2002graph,
	title={Introduction to graph theory},
	author={D. B. West},
	edition={2},
	year={2001},
	publisher={Prentice Hall}
}
@article{patil2020zero,
  title={Zero-divisor graph of a poset with respect to an automorphism},
  author={Patil, Avinash and Khairnar, Anil and Waphare, BN},
  journal={Discrete Appl. Math.},
  volume={283},
  pages={604--612},
  year={2020},
  publisher={Elsevier}
}

@article{khairnar2016zero,
  title={Zero-Divisor Graphs of Laurent Polynomials and Laurent Power Series},
  author={Khairnar, Anil and Waphare, BN},
  booktitle={J. Algebra its Appl.},
  pages={345--349},
  year={2016},
  publisher={Springer}
}
@article{Jitsupat2021eigenvalues,
	title={Eigenvalues of zero divisor graphs of principal ideal rings},
	author={Jitsupat Rattanakangwanwong and Yotsanan Meemark},
	journal={Linear Multilinear Algebra},
	volume={70},
	number={20},
	pages={5445--5459},
	year={2022},
	publisher={Taylor and Francis}
}

\end{document}




@article{pirzada2023signless,
  title={Signless Laplacian eigenvalues of the zero divisor graph associated to finite commutative ring $ mathbb $\{$Z$\}$ \_ $\{$p\^{}$\{$M\_ $\{$1$\}$$\}$ q\^{}$\{$M\_ $\{$2$\}$$\}$$\}$ $},
  author={Pirzada, Shariefuddin and Rather, Bilal and Shaban, Rezwan Ul and Chishti, Tariq},
  journal={Communications in Combinatorics and Optimization},
  volume={8},
  number={3},
  pages={561--574},
  year={2023},
  publisher={Azarbaijan Shahid Madani University}
}

